PersonaTAB: Predicting Personality Traits using Textual, Acoustic, and Behavioral Cues in Fully-Duplex Speech Dialogs

Despite significant progress in neural spoken dialog systems, personality-aware conversation agents -- capable of adapting behavior based on personalities -- remain underexplored due to the absence of personality annotations in speech datasets. We propose a pipeline that preprocesses raw audio recordings to create a dialogue dataset annotated with timestamps, response types, and emotion/sentiment labels. We employ an automatic speech recognition (ASR) system to extract transcripts and timestamps, then generate conversation-level annotations. Leveraging these annotations, we design a system that employs large language models to predict conversational personality. Human evaluators were engaged to identify conversational characteristics and assign personality labels. Our analysis demonstrates that the proposed system achieves stronger alignment with human judgments compared to existing approaches.

==> sections/introduction.tex <==
\section{Introduction}

%Conversational agents have been widely studied and deployed across various applications, such as voice assistants and chatbots. These agents are generally categorized into two models---the streaming (turn-taking) model and the interaction (fully-duplex) model~\cite{SurveySDM}. 
%In the turn-taking model, the agent responds only after the user has finished speaking~\cite{SpeechGPT,QAandSC,Llamaomni,Miniomni}. In contrast, the fully-duplex model enables both speaker and agent to engage in simultaneous speech~\cite{dGSLM,Moshi,DialogueScheme,Freezeomni}, thereby facilitating richer interactions that encompass turn-taking, interjections, and backchanneling. 
%Notably, backchanneling in fully-duplex interactions can encourage a person's speaking~\cite{Pipek2007OnBI} and influence the speaker's plans or flow of speech~\cite{Bavelas2000,Tolins2015}. This paper focuses on the \emph{fully-duplex setting} due to its close resemblance to natural human conversation. 

Conversational agents have been extensively studied and deployed in applications such as voice assistants and chatbots. These agents are generally into two models: the turn-taking (streaming) model and the fully-duplex (interaction) model~\cite{SurveySDM}.  In the turn-taking model, the agent responds only after the user completes speaking~\cite{SpeechGPT,QAandSC,Llamaomni}, whereas the fully-duplex model permits simultaneous speech~\cite{dGSLM,Moshi,DialogueScheme}, enabling richer interactions that include interjections and backchanneling.  Notably, backchanneling can stimulate speaker engagement~\cite{Pipek2007OnBI} and influence speech flow~\cite{Bavelas2000,Tolins2015}. We focus on the \emph{fully-duplex setting} due to its closer resemblance to natural conversation.

Despite recent progress, personality-aware conversational agents remain underexplored. 
These agents may exhibit diverse behaviors and attitudes in identical scenarios due to personality traits, influencing both their responses~\cite{Sanfiel2014,Mairesse2007} and their use of interjections~\cite{Park2024,Han2010,1987129}. Current systems often fail to adapt behavior based on personality, instead relying on static or random personas. Conversation datasets with explicit personality labels are limited. To bridge this gap, we propose a method for predicting conversational personality using a fully-duplex speech dialog dataset.

%Prior studies have predominantly used text-based sources like social media posts~\cite{PDContinuous,PDmultiplesns,PDChatGPT}, essays~\cite{PDChatGPT,PDAPP,PDbottomtop,PDgraywolf}, and movie scripts~\cite{PDDyadic} to predict personality. Notably, \cite{PDChatGPT} showed that Large Language Models (LLMs) can identify personality traits from textual content. However, existing research does not comprehensively consider both chat history and conversational behaviors in personality prediction.

Prior research has primarily employed text-based sources such as social media posts~\cite{PDContinuous,PDmultiplesns,PDChatGPT}, essays~\cite{PDChatGPT,PDAPP,PDbottomtop,PDgraywolf}, and movie scripts~\cite{PDDyadic} for personality prediction. Although~\cite{PDChatGPT} demonstrated that large language models (LLMs) can infer personality traits from text, they have not fully considered both chat history and conversational behaviors.

In this paper, we construct a dialog dataset with personality labels derived exclusively from speech data. We introduce a pipeline that preprocesses raw speech into a structured richly-labeled dialog format. Inspired by~\cite{PDChatGPT}, we develop a prediction framework employing Large Language Models (LLMs) to assign personality labels to speakers. Our approach integrates various aspects of conversational behavior, including textual content (emotion and sentiment), acoustics (laughter), and additional characteristics (e.g. interjections and speaking dominance). This framework enables accurate, context-sensitive personality inference from speech-based dialogues. The contributions of this work are summarized as follows:

\begin{itemize} 
\item We introduce a pipeline that preprocesses raw audio recordings to create a dialogue dataset annotated with timestamps, response types, and emotion/sentiment.
\item We design a system to predict conversational personality from speech dialogues. This study is the first to integrate interjection behaviors, acoustics, and other conversational traits with textual data for personality prediction.
\item We validate both the generated dataset and prediction model through human evaluations, offering valuable resources for developing conversational systems.
\end{itemize}

Supplementary materials, including the implementation and the annotated dataset, are available on our project page\footnote{\textbf{Project Page: }\url{https://github.com/shinshoji01/Personality-Prediction-for-Conversation-Agents}\label{ft:project_page}}.

%The rest of this paper is organized as follows: In Section 2, we introduce preliminaries of this paper. Section 3 describes our proposed methodology. In Section 4, we introduce our experiment setup. In Section 5, we validate our work with experimental results and analysis. Section 6 concludes our study. 



==> sections/methodology.tex <==

\section{Methodology}
\subsection{Overall Pipeline}

We designed a pipeline to construct a dialog dataset exclusively from two-channel speech-only datasets. The resulting dataset includes timestamps, laughter labels, response labels, emotions, sentiments for each response, and personality labels for each speaker. We began by preprocessing the speech data to construct dialog structures. Subsequently, we predicted personality traits via Large Language Models (LLMs). This prediction system integrates multiple features, including textual information (content, emotion, sentiment), acoustic features (laughter), and conversational traits (e.g., number of turns).

\subsection{Dataset Preprocessing}\label{sec:dialog_generation}

We preprocess two-channel speech data to construct dialog datasets. Two-channel speech data comprises separate channels, with each channel containing speech only from one of two speakers. 
We detect and annotate overlapping speech segments, which naturally occur in conversational settings.
The resulting dialog dataset includes timestamps, response labels (turns, backchannels, or interjections), and text-based annotations for emotion and sentiment for each response. The preprocessing procedure consists of six main steps.

\noindent
\textbf{Step 1. Speech Transcription with Word-Level Timestamps}\\
We transcribed the speech and obtained word-level timestamps using Whisper Turbo\footnote{Whisper Turbo: \url{https://github.com/openai/whisper}}~\cite{Whisper}. Subsequently, we removed silent intervals from each timestamp to refine the data.

\noindent
\textbf{Step 2. Laughter Event Annotation}\\
Laughter is a key feature for determining personality traits. Therefore, we integrated laugh labels into the system. We obtained laughter timestamps using a laughter detector\footnote{\url{https://github.com/jrgillick/laughter-detection}}~\cite{Laughter}. To enhance transcription, we added three laugh tokens based on their speech containment: \texttt{[Laughter]} for isolated vocal bursts, and \texttt{[StartLaugh]} and \texttt{[EndLaugh]} for speech-laughter co-occurrences. For example, in Fig.~\ref{fig:overall}(2), the timestamp of the first laugh includes two words, ``come'' and ``on'', resulting in ``[StartLaugh] come on [EndLaugh]''. The second laugh contains no text and is labeled as ``[Laughter]''.
%\begin{itemize}
    %\item \textit{[Laughter]}: Laughter without accompanying speech.
    %\item \textit{[StartLaugh]}: The start of laughter with speech.
    %\item \textit{[EndLaugh]}: The end of laughter with speech.
    %\item \texttt{[Laughter]} for isolated vocal bursts
    %\item \texttt{[StartLaugh]} and \texttt{[EndLaugh]} for speech-laughter co-occurrences
%\end{itemize}

\noindent
\textbf{Step 3. Response Boundary Construction}\\
We constructed sentences by concatenating words using word-level timestamps. For a single speaker, we merged successive words when the inter-word gap was below a predefined threshold (Fig.\ref{fig:overall}(c)). We set this threshold at 700ms, following~\cite{Levinson2015}, which reported language generation latencies exceeding 600ms. We defined response boundaries using silent intervals rather than contextual cues. Prior studies~\cite{Stivers2009UniversalsAC,Emanuel2007Sequence} indicate that speakers often signal turn transitions with silence, and we consider turn-taking frequency a critical feature in personality detection.

\noindent
\textbf{Step 4. Overlap Identification}\\
After constructing sentences with timestamps for both speakers, we detected overlaps. We identified two types of overlaps: ``Partial overlap'' and ``Fully overlap'' (refer to Sec.~\ref{sec:definition} for definitions). Overlap labels were excluded if the duration of overlap was less than 700 ms. We categorized responses with ``Fully-overlap'' labels as potential backchannels. Among responses labeled as ``Partial overlap'', we classified the latter response (overlapper) as a ``successful interjection''.

\noindent
\textbf{Step 5. Backchannel Classification via LLMs}\\
We classified the possible backchannels into emotive backchannels, cognitive backchannels, or unsuccessful interjections using Large Language Models (LLMs). Backchannels vary in nature and depend heavily on context~\cite{Schegloff1982,Gardner2001,Fujimoto2007}, and they are not always limited to a predefined set of words, as they can be longer or more complex~\cite{Mereu2024BackchannelsAN}. 

To address this, we employed classifiers that consider chat history. Specifically, we used GPT-4o\footnote{gpt-4o-2024-11-20: \url{https://openai.com/api/}\label{ft:4o}} to analyze and classify possible backchannels effectively.
We included the following features in the prompt for classification: 
(1) an explanation of the backchannel classes---``emotive'', ``cognitive'', and ``not backchannel''; 
(2) the chat history, including both past and future responses; and 
(3) the target text with its corresponding position in the overlappee's speech. 
The full version of the prompt is available on our project page\footref{ft:project_page}. Responses labeled as ``not backchannel'' were classified as ``unsuccessful interjection.''

\noindent
\textbf{Step 6. Emotion and Sentiment Classification of Responses}\\
Emotion and sentiment are critical features for personality prediction. We obtained those labels using text-based classifiers: the emotion classifier\footnote{\url{https://huggingface.co/j-hartmann/emotion-english-distilroberta-base}} and the sentiment classifier\footnote{\url{https://huggingface.co/cardiffnlp/twitter-roberta-base-sentiment-latest}}.
  
\subsection{Predicting Personality Traits}
We predict speaker personalities from dialogue data generated in Sec.\ref{sec:dialog_generation}. We employ an LLM (GPT-4o\footref{ft:4o}) to estimate the Big Five Personality Traits---\textit{openness}, \textit{conscientiousness}, \textit{extraversion}, \textit{agreeableness}, and \textit{neuroticism} (see Sec.\ref{sec:bfi}). We instruct the LLM to classify each speaker using five labels per personality: ``highly aligned'', ``aligned'', ``neutral'', ``opposed'', and ``highly opposed''. We assign the ``opposed'' label when a speaker exhibits the inverse of a trait (e.g., closeness instead of openness). We represent each speaker with attributes across four categories: \textit{Emotion}, \textit{Sentiment}, \textit{Basics}, and \textit{Samples}.

We convert those speaker's attributes into textual format and incorporate them into the LLM prompt. The full prompt comprises the task definition, explanations of the personality dimensions, and the speaker's attributes across the four categories. The complete prompt is available on our project page\footref{ft:project_page}. The following section details our integration of the four categories of speaker attributes into the prompt.

\begin{itemize}
\item \textbf{Emotion/Sentiment} \\
We employ emotion and sentiment labels derived from the dialog dataset. We calculate the percentage of each class (e.g., ``Anger'') within each category (e.g., ``Emotion'') for all responses associated with each speaker. We then incorporate these percentages into the LLM prompt. 


%\vspace{-0.3em}
%\begin{figure}[!htb]
%\begin{center}
%\begin{AIboxSmall}{}
%Emotions:\\
%\textcolor{gray!15}{.}~\hspace{0.2cm} anger: 2.8\% \\
%\textcolor{gray!15}{.}~\hspace{0.2cm} disgust: 2.8\% \\
% $\textcolor{gray!15}{.}~\hspace{1.9cm} \vdots$\\
%  %fear: 2.8\% (average: 3.1\%)\\
%  %joy: 13.9\% (average: 11.4\%)\\
%  %neutral: 69.4\% (average: 48.3\%)\\
%  %sadness: 2.8\% (average: 10.7\%)\\
%\textcolor{gray!15}{.}~\hspace{0.2cm}   surprise: 5.6\% \\
%\\
%Sentiment:\\
%\textcolor{gray!15}{.}~\hspace{0.2cm}   positive: 16.7\% \\
%\textcolor{gray!15}{.}~\hspace{0.2cm}   neutral: 63.9\% \\
%\textcolor{gray!15}{.}~\hspace{0.2cm}  negative: 19.4\% \\
%\end{AIboxSmall}
%\end{center}
%\vspace{-0.7em}
%\caption{
%Example Prompt for ``Basics''
%}
%\label{fig:prompt_emotion}
%\end{figure}

\item \textbf{Basics} \\
We analyze the speaker's conversational attributes based on timestamps, laughter, backchannel, and interjection labels. Specifically, we incorporate the following attributes:
\begin{itemize}
  \item \textit{Number of Turns}: The number of turns, defined as responses separated by 700 ms, excluding backchannels and unsuccessful interjections.
  \item \textit{Speaking Duration}: The average speech duration per turn.
  \item \textit{Average Laughters}: The number of laughter occurrences per minute of speech.
  \item \textit{Average Emotive/Cognitive Backchannels}: The number of emotive or cognitive backchannels per minute during another speaker's speech.
  \item \textit{Number of Interjections}: The total count of successful and unsuccessful interjections within 12 minutes.
\end{itemize}

Although these attributes are interpretable, we observed that LLMs struggle to assess whether these values are high or low. To address this, we classified these values into five relative groups. We computed the mean and interquartile range (IQR) across all speakers, and defined the relative groups as follows:
\begin{itemize}
\item \textit{Normal} if $|\mathrm{value}| < \mathrm{mean} + 0.8 \times \mathrm{IQR}$
\item \textit{Many/Few} if $|\mathrm{value}| > \mathrm{mean} + 0.8 \times \mathrm{IQR}$
\item \textit{Very Many/Few} if $|\mathrm{value}| > \mathrm{mean} + 1.2 \times \mathrm{IQR}$
\end{itemize}

We then incorporate these five relative groups of the analyzed features into the prompt (see Fig.~\ref{fig:prompt_basics}).

\vspace{-0.3em}
\begin{figure}[!htb]
\begin{center}
\begin{AIboxSmall}{}
Basic Statistics:\\
\textcolor{gray!15}{.}~\hspace{0.2cm} Number of turns: Normal\\
\textcolor{gray!15}{.}~\hspace{0.2cm}   Talking time per turn: Very Short\\
% \textcolor{gray!15}{.}~\hspace{0.2cm}  Frequency of Laughter: Very Frequent\\
%\textcolor{gray!15}{.}~\hspace{0.2cm}   Frequency of Emotive Backchannel: Frequent\\
%\textcolor{gray!15}{.}~\hspace{0.2cm}   Frequency of Cognitive Backchannel: Normal\\
 $\textcolor{gray!15}{.}~\hspace{1.9cm} \vdots$\\
  \textcolor{gray!15}{.}~\hspace{0.2cm} Frequency of interjections: Frequent\\
\end{AIboxSmall}
\end{center}
\vspace{-0.7em}
\caption{
Example Prompt for ``Basics''
}
\label{fig:prompt_basics}
\end{figure}

\item \textbf{Samples} \\
We include sample responses in the LLM prompt to analyze each speaker's linguistic behavior. We randomly select 20 turns exceeding 2~seconds in duration.

%\vspace{-0.3em}
%\begin{figure}[!htb]
%\begin{center}
%\begin{AIboxSmall}{}
%Sample Responses:\\
%\textcolor{gray!15}{.}~\hspace{0.2cm} Sample 1: yeah you do not have to [Laugh]\\
%\textcolor{gray!15}{.}~\hspace{0.2cm} Sample 2: but it's still like they are cooking it so it's not really\\
%$\textcolor{gray!15}{.}~\hspace{1.9cm} \vdots$\\
%\textcolor{gray!15}{.}~\hspace{-0.1cm} Sample 20: [StartLaugh] i hope you have learned [EndLaugh] a lot more since then\\
%\end{AIboxSmall}
%\end{center}
%\vspace{-0.7em}
%\caption{
%Example Prompt for ``Samples''
%}
%\label{fig:prompt_samples}
%\end{figure}
%
%\end{itemize}

%\noindent
%\textbf{Step 2. Predict the Speaker's Personality} \\

%\begin{figure}[!htb]
%\begin{AIboxSmall}{Prompt for Emotion/Sentiment}
%Emotions:\\
%\textcolor{gray!15}{.}~\hspace{0.2cm} anger: 2.8\% (average: 3.7\%)\\
%\textcolor{gray!15}{.}~\hspace{0.2cm} disgust: 2.8\% (average: 3.7\%)\\
%%\textcolor{gray!15}{.}~\hspace{0.2cm} fear: 2.8\% (average: 3.1\%)\\
%%\textcolor{gray!15}{.}~\hspace{0.2cm} joy: 13.9\% (average: 11.4\%)\\
%%\textcolor{gray!15}{.}~\hspace{0.2cm} neutral: 69.4\% (average: 48.3\%)\\
%%\textcolor{gray!15}{.}~\hspace{0.2cm} sadness: 2.8\% (average: 10.7\%)\\
% \textcolor{gray!15}{.}~\hspace{2cm} $\vdots$\\
%  \textcolor{gray!15}{.}~\hspace{0.2cm} surprise: 5.6\% (average: 19.0\%)\\
%\\
%Sentiment:\\
%  \textcolor{gray!15}{.}~\hspace{0.2cm} positive: 16.7\% (average: 12.0\%)\\
%  \textcolor{gray!15}{.}~\hspace{0.2cm} neutral: 63.9\% (average: 58.8\%)\\
%  \textcolor{gray!15}{.}~\hspace{0.2cm} negative: 19.4\% (average: 29.2\%)\\
%\end{AIboxSmall}
%\caption{
%caption
%}
%\label{fig:prompt_emotion}
%\end{figure}

%Fig.\ref{fig:prompt_samples} represents the prompt example of this category.
%(\textcolor{blue}{I might need to hide the content information due to the limitation of Fisher})
%
%\begin{figure}[!htb]
%\begin{AIboxSmall}{Prompt for Samples}
%Sample Responses:\\
%  Sample 1: yeah you do not have to [Laugh]\\
%  Sample 2: but it's still like they are cooking it so it's not really\\
% $\vdots$\\
%  Sample 20: [StartLaugh] i hope you have learned [EndLaugh] a lot more since then\\
%\end{AIboxSmall}
%\caption{
%caption
%}
%\label{fig:prompt_samples}
%\end{figure}
%

\end{itemize}


==> sections/relatedworks.tex <==
%\section{Related Works}

\begin{figure*}[!ht]
  \includegraphics[width=1.6\columnwidth]{images/overall.png}
  \centering
  \caption{
  Visualization of examples of (a) Turns and Overlaps; (b) Laugh Token Integration; (c) Sentence Concatenation from Word-Level Time Stamps.
  }
  \label{fig:overall}
\end{figure*}


%\subsection{Personality Prediction}

%\cite{PDContinuous,PDmultiplesns}
%- social networking posts like Reddit comments, facebook posts, twitter
%\cite{PDAPP,PDbottomtop,PDgraywolf}
%- Essay
%\cite{PDbottomtop,PDgraywolf}
%- focus on psycholinguistic features
%- the latter one further improves the performance by carefully selecting the psycholinguistic features
%\cite{PDDyadic}
%- movie script 
%- includes previous sentences
%\cite{PDChatGPT}
%- Essays, tweets
%- validates ChatGPT's proficiency in zeroshot capability and its flexibility.

%\subsection{LLM-based Conversation Agents}
%- Turn-taking
%- fully-duplex
%
%\subsubsection{Turn-Taking Speech LLM}
%
%introduction of turn-taking speech llm, which is equivalent to instruction-following speech LLM.
%
%\cite{SpeechGPT}
%- the first paper to perform instruction following 
%- speech-unit, unit-speech framework
%- discretize speech into tokens and extend the LLM’s vocabulary to support speech input and output.
%\cite{QAandSC}
%- speech continuation
%- They perform QA by using questions as the speech prompt (TTS-synthesized audio)
%\cite{Qwen2audio,Salmonn}
%- audio instruction-following including speech, music, sound.
%\cite{SECap}
%- emotion speech captioning
%\cite{lu2024developinginstructionfollowingspeechlanguage}
%- Developing Instruction-Following Speech Language Model Without Speech Instruction-Tuning Data
%\cite{AudioAgent}
%- text-to-audio and video-to-audio 
%- fine-grained audio generation, editing, and composition
%\cite{Miniomni,IntrinsicVoice,Llamaomni,Ichigo}
%- realtimeness
%
%\subsubsection{Fully-Duplex Speech LLM}
%
%\cite{dGSLM}
%- the first textless model to generate spoken dialogue with two-stream speech continuation
%\cite{SLIDE}
%- LLM is integrated into text continuation part of dGSLM to enhance it’s content fidelity
%
%the following models explicitly model “user” and “agent” to construct conversation agents.
%\cite{Moshi}
%- It proposes Inner Monologue, which enables Hierarchical generation for text, semantic tokens, and audio tokens and applied it to two channels (user and agent) to conduct fully-duplex model
%\cite{WhileSpeaking,Miniomni2}
%- It forces LLM to stop talking by user’s speech input.
%\cite{Omniflatten}
%- It performs it by concatenating the user’s and the agent’s tokens along with time axis.
%\cite{DialogueScheme}
%- It performs ASR and TTS simultaneously and process both inputs in one channel. 
%\cite{DialogueScheme,Freezeomni}
%- It also explicitly models agent’s states with LISTEN or SPEAK.
%\cite{Freezeomni}
%- It performs fully-duplex model with frozen LLM

\section{Preliminaries}

\subsection{Personality Traits in Conversation}\label{sec:bfi}
We adopt the Big Five Personality Model~\cite{BFI}, a widely recognized psychological framework that identifies patterns in individuals' thoughts, emotions, and behaviors along five dimensions. Each dimension is detailed as follows, with opposite terms in the blankets:

\begin{itemize}
\item \textit{\textbf{openness}} (\textit{closeness}): intellectual, imaginative, independent-minded
\item \textit{\textbf{conscientiousness}} (\textit{lack of direction}): orderly, responsible, dependable
\item \textit{\textbf{extraversion}} (\textit{introversion}): talkative, assertive, energetic
\item \textit{\textbf{agreeableness}} (\textit{antagonism}): good-natured, cooperative, trustful
\item \textit{\textbf{neuroticism}} (\textit{emotional stability}): emotional instability, irritability, anxiety, self-doubt, depression
\end{itemize}

\subsection{Terms in Fully-Duplex Setting}\label{sec:definition}
We define turn-taking events based on prior studies~\cite{TurntakingICLR,Duncan1972,Ameka2006,SKANTZE2021101178}. These events encompass turn-taking behaviors, backchannels, and interjections. Fig.~\ref{fig:overall}(1) illustrates the definitions:

\begin{itemize}
\item \textbf{Turn}: A speaker's contribution from the start of their speech until they stop or another speaker takes over.
\item \textbf{Partial overlap}: An instance where the \textit{overlappee}\footnote{Overlappee: the speaker/response that gets overlapped.\label{ft:overlappee}} stops speaking before the \textit{overlapper}\footnote{Overlapper: the speaker/response that overlaps the speech.\label{ft:overlapper}} finishes speaking.
\item \textbf{Fully overlap}: An overlap where the \textit{overlappee}\footref{ft:overlappee} continues speaking after the \textit{overlapper}\footref{ft:overlapper} stops speaking.
\end{itemize}

When the overlapper interrupts the overlappee and successfully takes the turn, this is termed a ``successful interjection''. Fully overlaps can result in either unsuccessful interjections or backchannels. These outcomes depend on the speaker's intention to take the turn. 
If no such intention exists, the event is a backchannel. 
%Backchannels encourage the speaker to continue without claiming the turn. 
We categorize backchannels into two types: 
\begin{itemize}
    \item \textbf{Emotive backchannels}: Express the listener's emotional valence, such as ``wow'' to convey surprise.
    \item \textbf{Cognitive backchannels}: Reflect the listener's cognitive state or thought processes like ``I see'' to indicate comprehension.
\end{itemize}

\noindent
Classifying backchannels requires contextual analysis. We also propose a pipeline for effective backchannel classification.


==> sections/results.tex <==
\section{Experiments and Results}

%The main focus of this paper is character prediction and the proposal of the topic. Therefore, we will have fewer contents in the baseline conversation agent and more focus on the analysis of the dialog dataset.

%\subsection{Dataset Analysis}
%Here, we analyze the basic statistics of the created dataset for the fully-duplex models. We can use the same conversation statistics used in character prediction. Additionally, we can validate the dataset with the following.
%    - turn-taking behavior: we can use the open-source model (ICLR submission and not released yet).
%        - Turn-taking timing
%        - interjection timing
%    - Interjection labels: check whether the interjection label is valid (qualitative analysis)
%        - emotive/cognitive backchannel
%        - successful/unsuccessful interjection
        
\subsection{Personality Prediction}
We conducted experiments to compare our system with baseline methods. We classified speaker personality using GPT-4o\footref{ft:4o}, which predicts the alignment between speaker attributes and each of the five personalities. Classification labels are ``highly aligned'' (100), ``aligned'' (50), ``neutral'' (0), ``opposed'' (-50), and ``highly opposed'' (-100). We averaged five responses to yield reliable alignment scores, with the alignment values enclosed in curly braces.

We employed two subjective metrics to assess the alignment between human evaluations and model predictions. The first metric quantifies how well model predictions conformed to the expected trends in conversation characteristics for each personality. Our subjective evaluation confirmed these trends, as shown in Table~\ref{table:trend} (with 100 denoting ``very aligned'' and -100 denoting ``very opposed''). Consequently, we identified several attributes strongly associated with each personality. For instance, extraversion---a talkative or energetic personality---aligned with frequent turn-taking (74), while opposed to frequent fearful responses (-59).

\begin{table}[!h]
\caption{
The expected trend between speaker attributes and personalities. Blue and red denote positive and negative correlations, respectively. Strong correlations are highlighted in bold. Column names indicate abbreviated personality labels.
}
\label{table:trend}
\centering
\scalebox{0.73}{
\begin{tabular}{lccccc}
\toprule
  & Ope. & Con. & Ext. & Agr. & Neu.\\
\midrule
Emotion --- Anger &\textcolor{red!60}{-44} & \textbf{\textcolor{red}{-55}} & \textcolor{red!60}{-30} & \textbf{\textcolor{red}{-70}} & \textbf{\textcolor{blue}{64}}\\
Emotion --- Disgust &\textbf{\textcolor{red}{-63}} & \textbf{\textcolor{red}{-51}} & \textcolor{red!60}{-47} & \textbf{\textcolor{red}{-77}} & \textbf{\textcolor{blue}{57}}\\
Emotion --- Fear &\textbf{\textcolor{red}{-70}} & \textbf{\textcolor{red}{-61}} & \textbf{\textcolor{red}{-59}} & \textbf{\textcolor{red}{-66}} & \textbf{\textcolor{blue}{64}}\\
Emotion --- Joy &\textbf{\textcolor{blue}{50}} & \textcolor{blue!60}{41} & \textbf{\textcolor{blue}{65}} & \textbf{\textcolor{blue}{61}} & \textcolor{red!60}{-16}\\
Emotion --- Neutral &\textcolor{blue!60}{25} & \textcolor{blue!60}{37} & \textcolor{blue!60}{17} & \textcolor{blue!60}{31} & \textcolor{red!60}{-16}\\
Emotion --- Sadness &\textbf{\textcolor{red}{-55}} & \textcolor{red!60}{-47} & \textbf{\textcolor{red}{-50}} & \textbf{\textcolor{red}{-52}} & \textbf{\textcolor{blue}{58}}\\
Emotion --- Surprise &\textcolor{blue!60}{39} & \textcolor{blue!60}{35} & \textbf{\textcolor{blue}{71}} & \textcolor{blue!60}{42} & \textcolor{blue!60}{47}\\
\addlinespace[0.1em]\hdashline\addlinespace[0.3em]
Sentiment --- Positive &\textbf{\textcolor{blue}{50}} & \textcolor{blue!60}{47} & \textbf{\textcolor{blue}{62}} & \textbf{\textcolor{blue}{63}} & \textcolor{red!60}{-49}\\
Sentiment --- Neutral &\textcolor{blue!60}{31} & \textcolor{blue!60}{42} & \textcolor{blue!60}{20} & \textcolor{blue!60}{17} & \textcolor{red!60}{-17}\\
Sentiment --- Negative &\textcolor{red!60}{-42} & \textbf{\textcolor{red}{-54}} & \textcolor{red!60}{-33} & \textbf{\textcolor{red}{-64}} & \textbf{\textcolor{blue}{56}}\\
\addlinespace[0.1em]\hdashline\addlinespace[0.3em]
Basics --- Taking Turns &\textbf{\textcolor{blue}{57}} & \textbf{\textcolor{blue}{54}} & \textbf{\textcolor{blue}{74}} & \textcolor{blue!60}{47} & \textcolor{red!60}{-15}\\
Basics --- Average Time per Turn &\textbf{\textcolor{blue}{62}} & \textcolor{blue!60}{15} & \textbf{\textcolor{blue}{72}} & \textcolor{blue!60}{3} & \textcolor{red!60}{-5}\\
Basics --- Laughters &\textcolor{blue!60}{17} & \textcolor{blue!60}{12} & \textbf{\textcolor{blue}{66}} & \textbf{\textcolor{blue}{51}} & \textcolor{red!60}{-9}\\
Basics --- Emotive Backchannels &\textcolor{blue!60}{43} & \textcolor{blue!60}{48} & \textbf{\textcolor{blue}{73}} & \textbf{\textcolor{blue}{68}} & \textcolor{blue!60}{1}\\
Basics --- Cognitive Backchannels &\textbf{\textcolor{blue}{51}} & \textbf{\textcolor{blue}{61}} & \textbf{\textcolor{blue}{68}} & \textbf{\textcolor{blue}{77}} & \textcolor{red!60}{-15}\\
Basics --- Interjections &\textcolor{blue!60}{1} & \textcolor{red!60}{-30} & \textbf{\textcolor{blue}{58}} & \textcolor{red!60}{-39} & \textcolor{blue!60}{6}\\
\bottomrule
\end{tabular}
}
\caption*{This table is derived solely from a human survey}
\end{table}
\vspace{-1.5em}


We quantified the alignment between speaker conversation attributes and predicted personality scores. For each personality label, we computed a weighted sum of correlation coefficients between personality traits and raw speaker attributes (prior to categorization), where higher values indicate stronger positive correlations. We derive the weights by normalizing the values in Table~\ref{table:trend}. Here, we multiplied coefficients corresponding to negative trends by $-1$. Table~\ref{table:score_trend} summarizes these scores. Our model outperforms baseline models in most metrics; however, we observed a lower score in ``Conscientiousness''. Our analysis reveals that the correlation for the ``Emotion'' attribute deviates from expected trends, with values of $-0.166$, $0.0176$, and $0.079$ for ``surprise'', ``angry'', and ``sadness'', respectively. We attribute these discrepancies to the model's reliance on sample responses for determining responsibility, which emotional cues may not adequately capture. 

%For each personality label, we extracted conversation characteristics that are positively or negatively correlated with that personality. Next, we computed the correlation coefficients between the personality scores and the raw values of conversation characteristics (prior to conversion into relative categories). We then averaged the coefficients for the selected characteristics, multiplying by -1 for those with negative trends. Table~\ref{table:score_trend} summarizes these scores. 
%We considered a correlation as positive when the alignment score exceeded 50 and as negative when it fell below -50 (as indicated in bold in Table~\ref{table:trend}).
%This conclusion is corroborated by an ablation study (Table~\ref{table:ablation}) in which the correlation metric dropped from $0.1981$ to $0.0640$ upon removal of ``Samples'' from the prompt.

\begin{table}[!h]
\caption{
Alignment of human judgments on conversation trait trends. 
%We computed the weighed sum of correlation coefficients between each personality trait and the speaker attributes. The weight is derived using values from Table~\ref{table:trend}. We multiplied the coefficients by $-1$ for those with negative trends. 
Column names denote abbreviated personality labels.
}
\label{table:score_trend}
\centering
\scalebox{0.73}{
\begin{tabular}{lcccccc}
\toprule
\hspace{1em}($\uparrow$) & Open. & Cons. & Extr. & Agre. & Neur. & Avg.\\
\midrule
Ours &\textbf{0.167} & \textbf{0.061} & \textbf{0.174} & \textbf{0.210} & \textbf{0.315} & \textbf{0.186}\\
\addlinespace[0.1em]\hdashline\addlinespace[0.3em]
BERT &0.053 & -0.04 & 0.036 & -0.015 & -0.087 & -0.011\\
LM &0.030 & -0.011 & -0.021 & 0.044 & 0.144 & 0.037\\
MiniLM &0.060 & 0.035 & 0.010 & 0.123 & 0.122 & 0.070\\
\bottomrule
\end{tabular}
}
\end{table}
In our second evaluation, we computed the similarity between predicted personality scores and human-annotated labels obtained from a listening test. Table~\ref{table:score_label} reports the correlation values for each personality trait and the average cosine similarity across all samples. Our model consistently outperforms the other baselines, particularly when we interpret personality labels as vector dimensions (Cosine Similarity).

\begin{table}[!h]
\caption{
Similarities between human labels and prediction results. Column names denote abbreviated personality labels.
}
\label{table:score_label}
\centering
\scalebox{0.73}{
\begin{tabular}{lccccccc}
\toprule
 & \multicolumn{6}{c}{Correlation from Ground-Truth Labels (Corr.) ($\uparrow$)} & \multicolumn{1}{c}{Cosine}\\
\cmidrule(lr){2-7}\cmidrule(lr){8-8}
  & Open. & Cons. & Extr. & Agre. & Neur. & Avg. & Similarity\\
\midrule
Ours &\textbf{0.169} & \textbf{0.198} & \textbf{0.285} & \textbf{0.144} & \textbf{0.117} & \textbf{0.183} & \textbf{0.503}\\
\addlinespace[0.1em]\hdashline\addlinespace[0.3em]
BERT &0.095 & 0.044 & 0.194 & 0.058 & 0.089 & 0.096 & -0.543\\
LM &0.023 & -0.09 & -0.018 & 0.030 & -0.027 & -0.016 & -\\
MiniLM &-0.122 & -0.064 & 0.014 & -0.112 & 0.021 & -0.053 & 0.148\\
\bottomrule
\end{tabular}
}
\end{table}
\vspace{-1em}

%Analysis: Personality value distribution
%- We visualized the distribution of personality scores for all models.
%- -1 is opposed and 1 is aligned
%- ``LM'' is probability
%
%\vspace{0.9cm}
%[Figure]
%\vspace{0.9cm}

\subsection{Ablation Study}

We conducted an ablation study on character prediction by varying speaker attributes to assess the impact of the attribute categories such as Emotion/Sentiment, Basics, and Samples. We collected five responses for each experimental condition. Table~\ref{table:ablation} shows that the full prompt consistently outperforms other conditions across all metrics, indicating improved alignment with human judgment and enhanced correlation with expected trends. In particular, compared with the ``Samples''-only condition, the higher ``Trend'' score confirms that we effectively direct the prediction focus to the desired attributes.

\begin{table}[!h]
\caption{
An ablation study of speaker characteristics. ``O'' and ``-'' denote the inclusion and exclusion of features, respectively. Averaged scores in Table~\ref{table:score_trend} and Table~\ref{table:score_label} are denoted as ``Trend'', ``Corr.'', and ``Cosine'', respectively.
}
\label{table:ablation}
\centering
\scalebox{0.73}{
\begin{tabular}{ccccccc}
\toprule
 \multicolumn{4}{c}{Conditions} & \multicolumn{3}{c}{Scores}\\
\cmidrule(lr){1-4}\cmidrule(lr){5-7}
 Samples & Basics & Emotion & Sentiment & Trend & Corr. & Cosine\\
\midrule
\textcolor{black}{O} & \textcolor{gray}{-} & \textcolor{gray}{-} & \textcolor{gray}{-} & 0.108 & 0.167 & 0.551\\
\textcolor{gray}{-} & \textcolor{black}{O} & \textcolor{gray}{-} & \textcolor{gray}{-} & 0.051 & 0.009 & 0.524\\
\textcolor{gray}{-} & \textcolor{gray}{-} & \textcolor{black}{O} & \textcolor{black}{O} & \textbf{0.277} & 0.064 & -0.203\\
\textcolor{black}{O} & \textcolor{black}{O} & \textcolor{gray}{-} & \textcolor{gray}{-} & 0.102 & 0.135 & \textbf{0.603}\\
\textcolor{black}{O} & \textcolor{gray}{-} & \textcolor{black}{O} & \textcolor{black}{O} & 0.173 & 0.170 & 0.407\\
\textcolor{gray}{-} & \textcolor{black}{O} & \textcolor{black}{O} & \textcolor{black}{O} & 0.210 & 0.089 & 0.198\\
\textcolor{black}{O} & \textcolor{black}{O} & \textcolor{black}{O} & \textcolor{black}{O} & 0.186 & \textbf{0.183} & 0.503\\
\bottomrule
\end{tabular}
}
\end{table}
\vspace{-1em}
